Lessons in Cooperation: A Qualitative Analysis of Driver Sentiments towards Real-Time Advisory Systems from a Driving Simulator User Study

Real-time Advisory (RTA) systems, such as navigational and eco-driving assistants, are becoming increasingly ubiquitous in vehicles due to their benefits for users and society. Until autonomous vehicles mature, such advisory systems will continue to expand their ability to cooperate with drivers, enabling safer and more eco-friendly driving practices while improving user experience. However, the interactions between these systems and drivers have not been studied extensively. To this end, we conduct a driving simulator study (N=16) to capture driver reactions to a Cooperative RTA system. Through a case study with a congestion mitigation assistant, we qualitatively analyze the sentiments of drivers towards advisory systems and discuss driver preferences for various aspects of the interaction. We comment on how the advice should be communicated, the effects of the advice on driver trust, and how drivers adapt to the system. We present recommendations to inform the future design of Cooperative RTA systems.

==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

In this section we provide an overview of works that implement and evaluate advisory systems and their interactions with drivers.
% Several works implement and evaluate advisory systems within vehicles for a multitude of application domains, including eco-driving, safe lane changes, and takeovers between autonomous and manual modes. 
% Here, we provide a broad overview of real-time advisory systems for vehicles in literature, with a particular focus on the eco-driving setting where our work lies.
% We additionally analyze the impacts of these systems on user trust, annoyance, cognitive load, and other factors.

% \subsection{Real-time Advisory Systems in Vehicles}

% Real-time advisory systems attempt to provide recommendations live to a user to accomplish an objective, as the surrounding environment evolves simultaneously.
% Two forms of real-time advisory systems commonly found in real vehicles include navigational assistants that provide directions to reach a goal location~\cite{bark2014personal,bolton2015investigation,nguyen2016efficient,obuhuma2018real}, and eco-driving modules that communicate ideal driving behavior to maximize fuel efficiency~\cite{chada2023evaluation,chada2022learning,chen2022driving,birrell2014effect,lin2014eco,lena2017vehicle}.
% % These types of systems are ubiquitous in vehicles in the form of navigational assistants that provide instructions to reach a goal location, and eco-driving instructions to maximize fuel efficiency.
% However, additional work has been undergone in the research community to develop and evaluate these types of systems in other areas, such as assisting drivers to make safe decisions~\cite{tran2013left,yan2016development,trabelsi2023advice,kim2016look}, and for influencing takeovers between an autonomous setting and manual control~\cite{kraus2016human,hock2016elaborating,large2019longitudinal,pakdamanian2022enjoy}.
% For example, in the research direction of safe advice,~\citet{tran2013left} provide information to drivers for making unprotected left turns through a heads-up display that visualizes the future path of oncoming vehicles for predicting a safe gap to turn into. Similarly,~\citet{yan2016development} detect when it is safe for a driver to change lanes and project recommendations onto the vehicle's side mirrors. 
% Within takeover scenarios,~\citet{large2019longitudinal} investigate the effectiveness of an autonomous vehicle and driver combination over a multi-day study, and identify that systems which ask users to check for hazards in the surroundings of the vehicle, before relinquishing control to the driver, improves driver readiness.
% % On the other hand,~\citet{hock2016elaborating} and~\citet{kraus2016human} rather propose to communicate with the driver to convince and prolong the vehicle control guided by the autonomous system 
% On the other hand,~\citet{hock2016elaborating} and~\citet{kraus2016human} investigate whether a communication module can delay the driver from taking control of the vehicle in a scenario where the autonomous setting may make safer decisions.
% Overall, researchers have showcased the promise of real-time advisory systems in vehicles in many settings.

\subsection{Evaluation of Real-time Eco-driving Advisory Systems}
% In this work, we analyze driver reactions to \sysacro~ systems through a case study on an eco-driving assistant in the form of traffic CM policies. 
% Here, we discuss popular eco-driving advisory systems and their methods of evaluation.
% In this work, we particularly evaluate driver reactions to real-time advisory systems for traffic congestion mitigation --- a form of eco-driving. 
% There is a vast set of works in literature that tackle providing real-time advice for eco-driving~\cite{asadi2011predictive, lin2014eco, fleming2021incorporating, chen2022driving, hasan2023perp, shahab2010auditory, birrell2014effect, lena2017vehicle, chada2022learning, chada2023evaluation, jayawardana2022ecolearning}.
Some eco-driving solutions forgo human-in-the-loop testing and rely completely on software simulations either due to limiting assumptions that render them hard to test or unsatisfactory performance in non-idealized settings~\cite{asadi2011predictive, lin2014eco, fleming2021incorporating, chen2022driving}.
Others such as \citet{birrell2014effect} test their solutions in expensive and potentially dangerous naturalistic studies, but only discuss the efficiency of their methods and its impact on user behavior without evaluating driver preferences on the interactions.
Meanwhile, driving simulator studies that address driver preferences have been conducted but only evaluate certain aspects of the user interface.
For example, \citet{shahab2010auditory} test the use of auditory modes to communicate how drivers should change their speeds based on pitch and \citet{lena2017vehicle} test the function of a \emph{gamified} UI.
Both works successfully show the validity of their UIs, but focus solely on the manner of communication and do not discuss driver preferences for either the systems' behaviors or the advice provided by such systems.
On the other hand, \citet{chada2023evaluation} test a novel CM system~\cite{chada2022learning} and capture quantitative metrics on the potential impact and user acceptance of CM system, but do not discuss qualitative opinions of drivers towards the tested \sysacro~ systems.
In contrast to these works, we first conduct human-in-the-loop driving simulator studies to allow participants to interact with \sysacro~ systems that exhibit a variety of behaviors.
We then conduct semi-structured interviews to understand the impact of the diverse behaviors on drivers and their perceptions to capture their preferences for their interactions with such systems.
We use these sentiments expressed by drivers to provide recommendations for the future \sysacro~ systems and discuss how their interactions can alter driver behavior.
% Some of these works make assumptions on the availability of sensor information that limit their adoption in practice. 
% For example,~\citet{asadi2011predictive} require knowledge of the state of traffic lights and~\citet{lin2014eco} design their method using a particular electric vehicle battery model that would need to be adapted to the actual deployment vehicle's model. 
% \citet{fleming2021incorporating} and~\citet{chen2022driving} introduce parameters that can be tuned to model driver preferences and traits, like following distance, cornering speed, and reaction time, but manually tuning these parameters may be expensive.
% Additionally, the advisory policies are developed with classical control methods that may perform poorly in scenarios the model was not designed to account for.
% On the other hand,~\citet{hasan2023perp} propose to estimate driver preferences and traits, and augment advice through learning-based methods that may generalize to unseen scenarios better than classical control approaches.
% While each of the preceding methods show promise in improving eco-driving goals, they limit their studies to simulated environments, and thus lack studies with real drivers.
% ~\citet{birrell2014effect} evaluate their Foot-LITE system, which provides advice on when to change gears, accelerate or brake, and warn about lane departures or tailgating, with real drivers on a fixed driving route in England.
% While the study led to relevant findings on how real-time advisory systems impact user behaviors, testing these systems on real roads is expensive and potentially dangerous.
% Furthermore, the study lacks discussion about the opinions of the drivers using the system.
% % \cheeloy{Mention here the one work that tests with drivers in a real car. It's expensive.}
% % As such, many researchers evaluate their eco-driving advisors with drivers in a car simulator.
% As such, a common practice in this research area is to evaluate advisory systems with drivers in a car simulator.
% For example, an early work from~\citet{shahab2010auditory} introduces an auditory system that produces sounds at different pitches to instruct a driver to change speeds.
% As constant tones may be uncomfortable to some drivers, some works instead rely on visual cues, dashboard icons, or speech to provide instructions.
% ~\citet{lena2017vehicle} propose a \emph{gamified} user interface that encourages eco-driving with achievements, badges, and persuasive feedback to the driver. 
% However, the authors only collect the opinions of participants in a focus group pertaining to the system's user interface, and leave combining the interface with a recommendation system to future work.
% One of the closest works to ours is from~\citet{chada2023evaluation}, who design a real-time eco-driving and safety assistant with a visual user interface, and evaluate it with real drivers in simulation --- analyzing both the impact of the system on driver behaviors, and the drivers' perceptions of the system itself. 
% Their method, however, requires knowledge of the traffic light states, does not adapt to driver traits, and uses a classical control method to communicate continuously changing speed instructions that may be hard to follow, as discussed by~\citet{pcp}.
% In an extension work,~\citet{chada2022learning} introduce a method of classifying driver traits with hierarchical cluster analysis, and augmenting eco-instructions based on said traits.
% However, their driver trait analysis is clustered into one of a few number of discrete models, whereas our method captures driver traits in a more expressive continuous space.
% Our policies also provide instructions for a constant period of time where they are unchanging, so that they are easier for drivers to follow.
% More technical details of the policies we test in this work is provided in our concurrent work\footnotemark[1].

% % % Eco-driving discussion

% % Simulation
% asadi2011predictive - uses traffic lights
% lin2014eco - dynamic programming using model of vehicle battery
% fleming2021incorporating - classical method (DP), incorporates driver preferences into model like IDM but lacks real-world study with users
% chen2022driving - classical method (MPC), compensates for reaction time but lacks real-world study with users
% hasan2023perp - learning-based method, augments advice based on predicted traits of driver lacks real-world study with users

% % User Study
% shahab2010auditory - simulator vehicle, beeps
% birrell2014effect - real car
% lena2017vehicle - gamification, focus group
% chada2022learning - discrete number of driver models, classical method (MPC), uses traffic lights, simulator vehicle
% chada2023evaluation - classical method (MPC), uses traffic lights, simulator vehicle, missing driver preferences, no hold time, analyzes both impact of system on driver, and driver's perception of system
% cite footnote


\subsection{Impacts on User Perception}

The introduction of real-time advisory systems in vehicles has prompted extensive research into their impacts on user perception, focusing on factors like trust, adoption, and cognitive load~\cite{Wilfinger2010Influences, ma2007effects, walch2017from, kraus2016human, Kraut2023AssertiveTR, Holthausen2019trust, Vongvit2022Meta, Helldin2013Presenting}. 
The interplay between trust and other psychological constructs, such as risk behavior and situation awareness, has been extensively studied, emphasizing that well-calibrated trust is essential for enhancing interactions with automated systems~\cite{Holthausen2019trust, Vongvit2022Meta}.
Trust in real-time advisory systems is influenced by their perceived reliability, transparency, and the user's understanding of system capabilities and limitations. Systems that provide consistent and accurate advice, along with explanations of their decisions, tend to be trusted more by users~\cite{Kraut2023AssertiveTR}. 
% Conversely, unexpected system behavior or lack of explanation can erode trust, particularly if the system's actions deviate from the user's expectations~\cite{Dixon2023Exploring}.
Additionally, the driving style of a system can significantly affect comfort, thereby impacting the overall user experience~\cite{Peng2023Exploring}.
User behavior and adoption intentions are heavily influenced by factors such as comfort, safety, cost, attractiveness, and driving enjoyment~\cite{Sadeghian2022Designing}.
% Factors like comfort, safety, cost, attractiveness, and driving enjoyment significantly influence user behavior and adoption intentions~\cite{Sadeghian2022Designing}.
Empirical studies have shown that users favor choice-based systems over manual ones for the sense of control they offer. Interestingly, trust in autonomous vehicles appears to mitigate the increase in driver-initiated takeovers as conflicts intensify, which suggests that user trust can play a pivotal role in the effective operation of these systems~\cite{Woide2023Ive}.
% Furthermore, systems that enhance safety or driving efficiency without introducing significant operational complexities are more likely to be embraced by users~\cite{lena2017vehicle}.
% Managing the cognitive load is also essential to prevent user overload and potential distractions. Systems that provide information in a clear, concise, and timely manner can help manage this load, thus maintaining driver focus and safety
Furthermore, systems that maintain safety or enhance driving efficiency without significant complexity are preferred, as they ease the cognitive burden on drivers. Clear, concise information delivery is key to managing cognitive load and maintaining driver safety~\cite{lena2017vehicle, kim2016look}.
In this work, by examining drivers' reactions and feelings towards the behavior of advisory systems, we seek to provide actionable insights that can enhance user-system interactions. These insights are aimed at fostering more favorable user experiences and broader acceptance of these technologies, focusing on real-world applicability and user-centric design.




% Considering these factors, the successful integration of advisory systems hinges on a balance between enhancing user experience and minimizing stress or complexity. Future research should further explore these dynamics through longitudinal studies to gain deeper insights into long-term user interactions with these systems~\cite{SrourZreik2023AgeMI}. % SrourZreik2023AgeMI is also at sae level 3

% Our research addresses previously identified gaps, such as inconsistencies between system advice and individual driving preferences, which had eroded trust and compliance. Our policies are designed to ensure that recommendations are not only easily understandable but also closely tailored to each driver's unique behavior and history, significantly enhancing trust and promoting long-term system engagement.


% Driver interactions with automation are known to have an effect on drivers perception of the automation in terms of trust





